ESNLIR: A Spanish Multi-Genre Dataset with Causal Relationships

Natural Language Inference (NLI), also known as Recognizing Textual Entailment (RTE), serves as a crucial area within the domain of Natural Language Processing (NLP). This area fundamentally empowers machines to discern semantic relationships between assorted sections of text. Even though considerable work has been executed for the English language, it has been observed that efforts for the Spanish language are relatively sparse. Keeping this in view, this paper focuses on generating a multi-genre Spanish dataset for NLI, ESNLIR, particularly accounting for causal Relationships. A preliminary baseline has been conceptualized and subjected to an evaluation, leveraging models drawn from the BERT family. The findings signify that the enrichment of genres essentially contributes to the enrichment of the model's capability to generalize. The code, notebooks and whole datasets for this experiments is available at: https://zenodo.org/records/15002575. If you are interested only in the dataset you can find it here: https://zenodo.org/records/15002371.

==> review_comment_status.tex <==
EMNLP

Reviewer #1
W1: Se necesita validar el corpus
W2: Escribir como se adapta SCINLI a espanol. SOLVED (Dataset 2.2)
W3: Providing examples (including even failure cases, based on validation of the data) would greatly improve the paper. SOLVED (Dataset 2.2) (Resultados 4.1)
W4: Error analysis of the provided baselines. SOLVED (Resultados 4.1)

Reviewer #2
W1: it is unclear how the data set was created. SOLVED (Dataset 2)
W2: No data validation is mentioned in the paper.
W3: The paper is missing some examples of the dataset. SOLVED (Dataset 2.2) (Resultados 4.1)
W4: The paper is missing any analysis of the model's performance (Resultados 4.1)

Reviewer #3
W1: The details of constructing the dataset are missing. SOLVED (Dataset 2)
W2: Experiments are weak.

- Since NLI only contains four labels, why select P/R/F1 for evaluation instead of traditional accuracy? (SOLVED 3.2 metrics saying it is balanced)
- Table 3 is confusing. Authors need to add results of other models (e.g., BERT) for comparison. And how do you get the 'Accuracy' here? Does it come from the average score of different label types (e.g., Contrasting, Neutral, etc)? (SOLVED se cambio la tabla por esta que si esta balanceada tab:performance)
- If so, it seems not reasonable since the data number for each label is different.
Do you check the cases in Table 4? It seems augmenting different genre data for training has the same results (all 0.67 in es_wiki_f1). Since the test dataset is quite large, the same results are weird. (SOLVED, para el paper de generalizacion, en este no va, y habia un bug de experimento que se corrigio el semestre pasado)



COLING

Reviewer #1
W1: Explicar la etiqueta reasoning soportado en la literatura. SOLVED (Explicacion de donde sale reasoning sacado y citando SCINLI 065-071)
W2: Explicar la etiqueta causal. SOLVED (Se explica en la TABLE {tab:classes}) 

W3: Mencionar que las evaluaciones las realizamos, pero consideramos deben ser objeto de otro paper. Adelantar que los resultados usando sobre nuestro dataset son peores que los BERT-base usando estado del arte como GPT4o. SOLVED (Limitations: 538-543)
W4: Previas revisiones nos mencionan que era mucho para un paper y que nos deberías enfocar en detallar la construcción del paper. Creo que es un tema subjetivo (SOLVED, INTRO, pero creo que se podria mejorar muchisimo si se resume el parrafo 2 y 3 de la Intro 041-100, ya que nombro el detalle de datasets anteriores pero como que es lo mismo una y otra vez).

Reviewer #2
-W1: Explicar reasoning.  SOLVED (TABLE {tab:classes})
-W2: Si puede introducir pero bias pero no necesariamente la clase neutral siempre tuvo un valor alto o si? SOLVED (Se puso una explicacion de que si se espera bias debido a que la forma de etiquetado es completamente diferente 200-206)
-W3: Agradecemos los comentarios y correjiremos los Typos. (PENDING, necesito ayuda por si hay algo que nos equivocamos GPT y yo)

Reviewer #3
-W1: Explorar con ESNLIR y INFERES. Se buscaron, pero no están disponible dichos datasets. Como respondemos el tema de calidad? (SOLVED 551-563)
-W2: No es solo general nuestro dataset, tambien tiene de ciencia, y hay que explicar esta etiqueta. SOLVED (Explicacion de donde sale reasoning sacado y citando SCINLI 065-071)
-W3:  BERTIN is a Roberta based model?, lo dice el paper correcto?.  Los resultados con LLMs los dejamos para un paper posterior. SOLVED (Cambio de RoBERTa a BERTIN, XLMRoBERTa si sigue igual)
